SMEFT Analysis of $m_{W}$

We use the Fitmaker tool to incorporate the recent CDF measurement of $m_W$ in a global fit to electroweak, Higgs, and diboson data in the Standard Model Effective Field Theory (SMEFT) including dimension-6 operators at linear order. We find that including any one of the SMEFT operators ${\cal O}_{HWB}$, ${\cal O}_{HD}$, ${\cal O}_{\ell \ell}$ or ${\cal O}_{H \ell}^{(3)}$ with a non-zero coefficient could provide a better fit than the Standard Model, with the strongest pull for ${\cal O}_{HD}$ and no tension with other electroweak precision data. We then analyse which tree-level single-field extensions of the Standard Model could generate such operator coefficients with the appropriate sign, and discuss the masses and couplings of these fields that best fit the CDF measurement and other data. In particular, the global fit favours either a singlet $Z^\prime$ vector boson, a scalar electroweak triplet with zero hypercharge, or a vector electroweak triplet with unit hypercharge, followed by a singlet heavy neutral lepton, all with masses in the multi-TeV range for unit coupling.

==> Ref_reply.tex <==
We thank the referee for finding our paper nice and useful and are happy to address concerns about the value of our analysis beyond the recent CDF measurement. To this end, we have noted in various places that previous measurements were already trending above the SM prediction, and that our analysis goes beyond previous SMEFT analyses by identifying flat directions in parameter space and analyzing the role of CKM unitarity.

Thus we have added a paragraph at the end of the introduction to summarise the value of our SMEFT analysis beyond the CDF measurement. We emphasize that there is much interest in the community to extend SMEFT fits globally as we have done in our previous study, and this analysis focusing on $M_W$ is a first step in taking our analysis framework towards the addition of other precision measurements such as CKM unitarity. Uncovering the flat directions in the Wilson coefficients helps to identify important measurements and their role. Moreover, our matching to single-field extensions singles out the relevant simplified models that these coefficients constrain. Such a systematic analysis helps to explore the space of BSM physics relevant in the $W$ mass measurement and other related physics, which were already of interest prior to CDF's latest update. 

As the referee suggested, we have enlarged the uncertainties of the CDF measurement according to the PDG prescription for combining data that are poorly consistent and shown how this affects the preferred ranges on the single-field extensions, as discussed in an expanded Section 4. This conservative procedure captures a hypothetical scenario where the CDF measurement is not as discrepant with other direct measurements but may still reflect an overall preference for slightly higher values. We note that the global fits in the past also found a mild pull towards higher values for the $W$ mass, so it may well be that future measurements converge away from the SM even if CDF under-represented their errors. 

Regarding the comment about single-field extensions, we considered only tree-level models matched to the SMEFT since the SMEFT approach may not be justified for loop-level models, which may well be excluded by direct searches. This is now mentioned at the beginning of Section 4. As the referee also suggests, we explicitly say in Section 3, at the beginning of the paragraph on the bottom of p. 8, that we are comparing indirect and direct measurements of the $W$ mass in the plots, and have added mention in the text and in the caption of Fig. 6 of the relevance of weak or strong couplings for the mass scales in the plot. 

We hope that, with these modifications highlighting the general value of our analysis independently of the fate of the CDF anomaly, our paper is suitable for publication. 

==> limit_table_old.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c||c|c|c|}
\hline
 & \multicolumn{3}{c||}{ Individual} & \multicolumn{3}{c|}{Marginalised} \\
 \hline
 SMEFT &  Best fit &   95\% CL &  Scale &  Best fit & 95\% CL &  Scale \\
 Coeff.   & [$\Lambda = 1$~TeV] & range & $\frac{\Lambda}{\sqrt{C}}$ [TeV] & [$\Lambda = 1$~TeV] & range & $\frac{\Lambda}{\sqrt{C}}$ [TeV] \\
\hline \hline
     $C_{HWB}$& 0.00 &[ -0.0043, +0.0026 ]& 17.0 & 0.18 &  [ -0.36, +0.73 ]  & 1.4  \tabularnewline\hline
      $C_{HD}$&-0.01 &[ -0.023, +0.0027 ] & 8.8  &-0.39 &  [ -1.6, +0.81 ]   & 0.91 \tabularnewline\hline
      $C_{ll}$& 0.01 & [ -0.005, +0.019 ] & 9.2  &-0.03 & [ -0.084, +0.02 ]  & 4.4  \tabularnewline\hline
$C_{Hl}^{(3)}$& 0.00 & [ -0.01, +0.003 ]  & 12.0 &-0.03 & [ -0.13, +0.055 ]  & 3.3  \tabularnewline\hline
$C_{Hl}^{(1)}$&0.00  &[ -0.0044, +0.013 ] & 11.0 & 0.11 &  [ -0.19, +0.41 ]  & 1.8  \tabularnewline\hline
      $C_{He}$& 0.00 &[ -0.015, +0.0071 ] & 9.6  & 0.19 &  [ -0.41, +0.79 ]  & 1.3  \tabularnewline\hline
$C_{Hq}^{(3)}$& 0.00 & [ -0.017, +0.012 ] & 8.3  &-0.05 & [ -0.11, +0.012 ]  & 4.1  \tabularnewline\hline
$C_{Hq}^{(1)}$& 0.02 &  [ -0.1, +0.14 ]   & 2.9  &-0.04 &  [ -0.27, +0.18 ]  & 2.1  \tabularnewline\hline
      $C_{Hd}$&-0.03 & [ -0.13, +0.071 ]  & 3.1  &-0.39 &  [ -0.91, +0.13 ]  & 1.4  \tabularnewline\hline
      $C_{Hu}$& 0.00 & [ -0.075, +0.073 ] & 3.7  &-0.19 &  [ -0.63, +0.25 ]  & 1.5  \tabularnewline\hline
    $C_{H\Box}$&-0.27 &   [ -1, +0.47 ]    & 1.2  & -0.9 &    [ -3, +1.2 ]    & 0.69 \tabularnewline\hline
      $C_{HG}$& 0.00 &[ -0.0034, +0.0032 ]& 17.0 & 0.00 &[ -0.014, +0.0086 ] & 9.4  \tabularnewline\hline
      $C_{HW}$& 0.00 & [ -0.012, +0.006 ] & 11.0 & 0.12 &  [ -0.38, +0.62 ]  & 1.4  \tabularnewline\hline
      $C_{HB}$& 0.00 &[ -0.0034, +0.002 ] & 19.0 & 0.07 &  [ -0.09, +0.22 ]  & 2.5  \tabularnewline\hline
       $C_{W}$& 0.18 & [ -0.071, +0.42 ]  & 2.0  & 0.15 &  [ -0.11, +0.4 ]   & 2.0  \tabularnewline\hline
       $C_{G}$&-0.46 &  [ -0.77, -0.14 ]  & 1.8  & -1.4 &  [ -2.2, -0.72 ]   & 1.2  \tabularnewline\hline
  $C_{\tau H}$& 0.01 & [ -0.015, +0.025 ] & 7.1  & 0.01 & [ -0.016, +0.028 ] & 6.7  \tabularnewline\hline
   $C_{\mu H}$& 0.00 &[ -0.0057, +0.005 ] & 14.0 & 0.00 &[ -0.0058, +0.005 ] & 14.0 \tabularnewline\hline
      $C_{bH}$&0.00  & [ -0.016, +0.024 ] & 7.1  & 0.01 & [ -0.034, +0.052 ] & 4.8  \tabularnewline\hline
      $C_{tH}$&-0.09 &   [ -1, +0.84 ]    & 1.0  & 1.5  &   [ -2.8, +5.7 ]   & 0.48 \tabularnewline\hline
\end{tabular}
}

==> m_W in the Standard Model Effective Field Theory/Ref_reply.tex <==
We thank the referee for finding our paper nice and useful and are happy to address concerns about the value of our analysis beyond the recent CDF measurement. To this end, we have noted in various places that previous measurements were already trending above the SM prediction, and that our analysis goes beyond previous SMEFT analyses by identifying flat directions in parameter space and analyzing the role of CKM unitarity.

Thus we have added a paragraph at the end of the introduction to summarise the value of our SMEFT analysis beyond the CDF measurement. We emphasize that there is much interest in the community to extend SMEFT fits globally as we have done in our previous study, and this analysis focusing on $M_W$ is a first step in taking our analysis framework towards the addition of other precision measurements such as CKM unitarity. Uncovering the flat directions in the Wilson coefficients helps to identify important measurements and their role. Moreover, our matching to single-field extensions singles out the relevant simplified models that these coefficients constrain. Such a systematic analysis helps to explore the space of BSM physics relevant in the $W$ mass measurement and other related physics, which were already of interest prior to CDF's latest update. 

As the referee suggested, we have enlarged the uncertainties of the CDF measurement according to the PDG prescription for combining data that are poorly consistent and shown how this affects the preferred ranges on the single-field extensions, as discussed in an expanded Section 4. This conservative procedure captures a hypothetical scenario where the CDF measurement is not as discrepant with other direct measurements but may still reflect an overall preference for slightly higher values. We note that the global fits in the past also found a mild pull towards higher values for the $W$ mass, so it may well be that future measurements converge away from the SM even if CDF under-represented their errors. 

Regarding the comment about single-field extensions, we considered only tree-level models matched to the SMEFT since the SMEFT approach may not be justified for loop-level models, which may well be excluded by direct searches. This is now mentioned at the beginning of Section 4. As the referee also suggests, we explicitly say in Section 3, at the beginning of the paragraph on the bottom of p. 8, that we are comparing indirect and direct measurements of the $W$ mass in the plots, and have added mention in the text and in the caption of Fig. 6 of the relevance of weak or strong couplings for the mass scales in the plot. 

We hope that, with these modifications highlighting the general value of our analysis independently of the fate of the CDF anomaly, our paper is suitable for publication. 

==> m_W in the Standard Model Effective Field Theory/limit_table.tex <==
\begin{tabular}{|c||c|c|c||c|c|c|}
\hline
 & \multicolumn{3}{c||}{ Individual} & \multicolumn{3}{c|}{Marginalised} \\
 \hline
 SMEFT &  Best fit &   95\% CL &  Scale &  Best fit & 95\% CL &  Scale \\
 Coeff.   & [$\Lambda = 1$~TeV] & range & $\frac{\Lambda}{\sqrt{C}}$ [TeV] & [$\Lambda = 1$~TeV] & range & $\frac{\Lambda}{\sqrt{C}}$ [TeV] \\
\hline \hline
     $C_{HWB}$&-0.01 &[ -0.009, -0.0034 ] & 19.0 & 0.25 &  [ -0.3, +0.81 ]   & 1.3  \tabularnewline\hline
      $C_{HD}$&-0.03 & [ -0.035, -0.019 ] & 11.0 & -0.6 &  [ -1.8, +0.63 ]   & 0.9  \tabularnewline\hline
      $C_{ll}$& 0.02 & [ +0.014, +0.034 ] & 10.0 &-0.05 &[ -0.099, +0.0043 ] & 4.4  \tabularnewline\hline
$C_{Hl}^{(3)}$&-0.01 &[ -0.019, -0.0083 ] & 14.0 &-0.01 & [ -0.11, +0.076 ]  & 3.3  \tabularnewline\hline
$C_{Hl}^{(1)}$&0.00  &[ -0.0045, +0.013 ] & 11.0 & 0.16 &  [ -0.15, +0.47 ]  & 1.8  \tabularnewline\hline
      $C_{He}$& 0.00 &[ -0.015, +0.0071 ] & 9.6  & 0.28 &  [ -0.34, +0.9 ]   & 1.3  \tabularnewline\hline
$C_{Hq}^{(3)}$& 0.00 & [ -0.013, +0.011 ] & 9.1  &-0.05 & [ -0.11, +0.012 ]  & 4.1  \tabularnewline\hline
$C_{Hq}^{(1)}$& 0.01 & [ -0.027, +0.043 ] & 5.4  &-0.07 &  [ -0.2, +0.06 ]   & 2.8  \tabularnewline\hline
      $C_{Hd}$&-0.03 & [ -0.13, +0.072 ]  & 3.1  &-0.44 & [ -0.96, +0.079 ]  & 1.4  \tabularnewline\hline
      $C_{Hu}$& 0.00 & [ -0.075, +0.073 ] & 3.7  &-0.18 &  [ -0.62, +0.26 ]  & 1.5  \tabularnewline\hline
    $C_{HBox}$&-0.27 &   [ -1, +0.47 ]    & 1.2  & -1.1 &    [ -3.2, +1 ]    & 0.69 \tabularnewline\hline
      $C_{HG}$& 0.00 &[ -0.0034, +0.0032 ]& 17.0 &-0.01 & [ -0.026, +0.013 ] & 7.2  \tabularnewline\hline
      $C_{HW}$& 0.00 & [ -0.012, +0.006 ] & 11.0 & 0.18 &  [ -0.33, +0.7 ]   & 1.4  \tabularnewline\hline
      $C_{HB}$& 0.00 &[ -0.0034, +0.002 ] & 19.0 & 0.09 & [ -0.074, +0.24 ]  & 2.5  \tabularnewline\hline
       $C_{W}$& 0.18 & [ -0.072, +0.42 ]  & 2.0  & 0.15 &   [ -0.1, +0.4 ]   & 2.0  \tabularnewline\hline
       $C_{G}$&-0.75 &    [ -4, +2.5 ]    & 0.56 & 1.3  &   [ -6.1, +8.7 ]   & 0.37 \tabularnewline\hline
  $C_{\tau H}$& 0.01 & [ -0.015, +0.025 ] & 7.1  &0.00  & [ -0.017, +0.027 ] & 6.7  \tabularnewline\hline
   $C_{\mu H}$& 0.00 &[ -0.0057, +0.005 ] & 14.0 & 0.00 &[ -0.0056, +0.0052 ]& 14.0 \tabularnewline\hline
      $C_{bH}$&0.00  & [ -0.016, +0.024 ] & 7.1  & 0.02 & [ -0.027, +0.058 ] & 4.8  \tabularnewline\hline
      $C_{tH}$&-0.09 &   [ -1, +0.84 ]    & 1.0  & -2.7 &   [ -8.8, +3.3 ]   & 0.41 \tabularnewline\hline
\end{tabular}



==> m_W in the Standard Model Effective Field Theory/limit_table_old.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c||c|c|c|}
\hline
 & \multicolumn{3}{c||}{ Individual} & \multicolumn{3}{c|}{Marginalised} \\
 \hline
 SMEFT &  Best fit &   95\% CL &  Scale &  Best fit & 95\% CL &  Scale \\
 Coeff.   & [$\Lambda = 1$~TeV] & range & $\frac{\Lambda}{\sqrt{C}}$ [TeV] & [$\Lambda = 1$~TeV] & range & $\frac{\Lambda}{\sqrt{C}}$ [TeV] \\
\hline \hline
     $C_{HWB}$& 0.00 &[ -0.0043, +0.0026 ]& 17.0 & 0.18 &  [ -0.36, +0.73 ]  & 1.4  \tabularnewline\hline
      $C_{HD}$&-0.01 &[ -0.023, +0.0027 ] & 8.8  &-0.39 &  [ -1.6, +0.81 ]   & 0.91 \tabularnewline\hline
      $C_{ll}$& 0.01 & [ -0.005, +0.019 ] & 9.2  &-0.03 & [ -0.084, +0.02 ]  & 4.4  \tabularnewline\hline
$C_{Hl}^{(3)}$& 0.00 & [ -0.01, +0.003 ]  & 12.0 &-0.03 & [ -0.13, +0.055 ]  & 3.3  \tabularnewline\hline
$C_{Hl}^{(1)}$&0.00  &[ -0.0044, +0.013 ] & 11.0 & 0.11 &  [ -0.19, +0.41 ]  & 1.8  \tabularnewline\hline
      $C_{He}$& 0.00 &[ -0.015, +0.0071 ] & 9.6  & 0.19 &  [ -0.41, +0.79 ]  & 1.3  \tabularnewline\hline
$C_{Hq}^{(3)}$& 0.00 & [ -0.017, +0.012 ] & 8.3  &-0.05 & [ -0.11, +0.012 ]  & 4.1  \tabularnewline\hline
$C_{Hq}^{(1)}$& 0.02 &  [ -0.1, +0.14 ]   & 2.9  &-0.04 &  [ -0.27, +0.18 ]  & 2.1  \tabularnewline\hline
      $C_{Hd}$&-0.03 & [ -0.13, +0.071 ]  & 3.1  &-0.39 &  [ -0.91, +0.13 ]  & 1.4  \tabularnewline\hline
      $C_{Hu}$& 0.00 & [ -0.075, +0.073 ] & 3.7  &-0.19 &  [ -0.63, +0.25 ]  & 1.5  \tabularnewline\hline
    $C_{H\Box}$&-0.27 &   [ -1, +0.47 ]    & 1.2  & -0.9 &    [ -3, +1.2 ]    & 0.69 \tabularnewline\hline
      $C_{HG}$& 0.00 &[ -0.0034, +0.0032 ]& 17.0 & 0.00 &[ -0.014, +0.0086 ] & 9.4  \tabularnewline\hline
      $C_{HW}$& 0.00 & [ -0.012, +0.006 ] & 11.0 & 0.12 &  [ -0.38, +0.62 ]  & 1.4  \tabularnewline\hline
      $C_{HB}$& 0.00 &[ -0.0034, +0.002 ] & 19.0 & 0.07 &  [ -0.09, +0.22 ]  & 2.5  \tabularnewline\hline
       $C_{W}$& 0.18 & [ -0.071, +0.42 ]  & 2.0  & 0.15 &  [ -0.11, +0.4 ]   & 2.0  \tabularnewline\hline
       $C_{G}$&-0.46 &  [ -0.77, -0.14 ]  & 1.8  & -1.4 &  [ -2.2, -0.72 ]   & 1.2  \tabularnewline\hline
  $C_{\tau H}$& 0.01 & [ -0.015, +0.025 ] & 7.1  & 0.01 & [ -0.016, +0.028 ] & 6.7  \tabularnewline\hline
   $C_{\mu H}$& 0.00 &[ -0.0057, +0.005 ] & 14.0 & 0.00 &[ -0.0058, +0.005 ] & 14.0 \tabularnewline\hline
      $C_{bH}$&0.00  & [ -0.016, +0.024 ] & 7.1  & 0.01 & [ -0.034, +0.052 ] & 4.8  \tabularnewline\hline
      $C_{tH}$&-0.09 &   [ -1, +0.84 ]    & 1.0  & 1.5  &   [ -2.8, +5.7 ]   & 0.48 \tabularnewline\hline
\end{tabular}
}
